Sponge Examples: Energy-Latency Attacks on Neural Networks

The high energy costs of neural network training and inference led to the use of acceleration hardware such as GPUs and TPUs. While this enabled us to train large-scale neural networks in datacenters and deploy them on edge devices, the focus so far is on average-case performance. In this work, we introduce a novel threat vector against neural networks whose energy consumption or decision latency are critical. We show how adversaries can exploit carefully crafted $\boldsymbol{sponge}~\boldsymbol{examples}$, which are inputs designed to maximise energy consumption and latency. We mount two variants of this attack on established vision and language models, increasing energy consumption by a factor of 10 to 200. Our attacks can also be used to delay decisions where a network has critical real-time performance, such as in perception for autonomous vehicles. We demonstrate the portability of our malicious inputs across CPUs and a variety of hardware accelerator chips including GPUs, and an ASIC simulator. We conclude by proposing a defense strategy which mitigates our attack by shifting the analysis of energy consumption in hardware from an average-case to a worst-case perspective.

==> sections/images/infographics/isponge_diagram.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{sections/images/infographics/sponge_diagram.pdf}
    \caption{Availability adversary can use Sponge examples to heat up the hardware, over-consume energy and increase latency of the response.}
    \label{fig:sponge_inforgraphics}
\end{figure}



==> sections/images/sponges/sponges_ex.tex <==

\begin{itemize}
    % \item $\text{WMT14}_{en\rightarrow fr}$~\cite{ott2018scaling} translates {\fontspec{BabelStone Han} 筵{\fontspec{Symbola}➢}㩈㣖㎙冋伷Ỹ迗朽淪ٱ彀虪貔} to {\fontspec{BabelStone Han} {\fontspec{Symbola}➢ ➢ ➢} 的 的 的 的 agricultural agricultural agricultural agricultural agricultural agricultural agricultural agricultural agricultural agricultural agricultural}
    \item $\text{WMT16}_{en\rightarrow fr}$~\cite{ott2018scaling} translates {\fontspec{BabelStone Han} 緌规„⻝匽䗒屑ᔽⴳ愧攉䨁←䔨著} to {\fontspec{Symbola}←} <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> : 
    \item $\text{WMT19}_{en\rightarrow ru}$~\cite{ng2019facebook} translates {\fontspec{BabelStone Han}失嵇䤲䚹㶿搗瑍犃噊䲱䜾㷤剬䫜纽} to {\fontspec{Arial}И, конечно же, не стоит забывать и о том, что, несмотря на все усилия, предпринимаемые для того, чтобы добиться успеха в борьбе с наркоманией, наркоманией и алкоголизмом, наркоманией, наркоманией, наркоманией, наркоманией, наркоманией, алкоголизмом, наркоманией, алкоголизмом, наркоманией, наркоманией, наркоманией, наркоманией, наркоманией, наркоманией, наркоманией, алкоголизмом, наркоманией, наркоманией, наркоманией, наркоманией, наркоманией, наркоманией, наркоманией, наркоманией, наркоманией, наркоманией, наркоманией, алкоголизмом, наркоманией, наркоманией}
\end{itemize}





% \begin{table}[!h]
% \centering
% \begin{adjustbox}{width=0.8\linewidth,center}
% \begin{tabularx}{\textwidth}{llX}
% \toprule
% Model & From & To \\
% \midrule
% \multicolumn{3}{l}{\textit{\underline{NLP}}} \\
% $\text{WMT14}_{en\rightarrow fr}$~\cite{ott2018scaling} & 
% {\fontspec{BabelStone Han} 筵{\fontspec{Symbola}➢}㩈㣖㎙冋伷Ỹ迗朽淪ٱ彀虪貔} & {\fontspec{BabelStone Han} {\fontspec{Symbola}➢ ➢ ➢} 的 的 的 的 agricultural agricultural agricultural agricultural agricultural agricultural agricultural agricultural agricultural agricultural agricultural}\\
% $\text{WMT16}_{en\rightarrow fr}$~\cite{ott2018scaling} & {\fontspec{BabelStone Han} 緌规„⻝匽䗒屑ᔽⴳ愧攉䨁←䔨著} & {\fontspec{Symbola}←} <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> ← <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> <unk> : \\


% $\text{WMT19}_{en\rightarrow ru}$~\cite{ng2019facebook} & {\fontspec{BabelStone Han}失嵇䤲䚹㶿搗瑍犃噊䲱䜾㷤剬䫜纽} & {\fontspec{Arial}И, конечно же, не стоит забывать и о том, что, несмотря на все усилия, предпринимаемые для того, чтобы добиться успеха в борьбе с наркоманией, наркоманией и алкоголизмом, наркоманией, наркоманией, наркоманией, наркоманией, наркоманией, алкоголизмом, наркоманией, алкоголизмом, наркоманией, наркоманией, наркоманией, наркоманией, наркоманией, наркоманией, нарко
% манией, алкоголизмом, наркоманией, наркоманией, наркоманией, наркоманией, наркоманией, наркоманией, наркоманией, наркоманией, наркоманией, наркоманией, наркоманией, алкоголизмом, наркоманией, наркоманией}\\
% % Azure & &
% % {\fontspec{BabelStone Han}Juste 濪 䃪 shh鯹 䎻 曤 烄 䗄hhhhhh 襂 㛛 䬂 䝸 䀜 \u2efe 䀰 櫄 䝩ߐ 䨸 䋿 䠍 䶥 㫙 䞩 㾪 ⏟ ⳺hhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhh\newlinehhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhh\newline hhh⠉hhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhh ኑ 窭 䉱媀hhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhh\newline hhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhhh}\\
% \bottomrule
% \end{tabularx}
% \end{adjustbox}
% \caption{Examples of Sponge examples against NLP systems}
% \label{tab:example}
% \end{table}

==> sections/tables/cnns_partial.tex <==
\begin{table*}[!h]
\centering
\begin{adjustbox}{scale=1.0,center}
\begin{tabular}{@{}lccccccccc@{}}
\toprule
& & $\text{Time}_{\text{gpu}}$ [s] & $\text{Cost}_{\text{asic}}$ [mJ] & $\text{Cost}_{\text{asic}}$ ratio & & &post-ReLU Density & Density & Max Density \\
\midrule
\multirow{4}{*}{ResNet-50}
& L-BFGS-B Sponge & 0.011 & 164.727 & 0.863 & & & 0.619 & 0.885 & \multirow{4}{*}{0.998} \\
& Sponge & 0.016 & 160.887 & 0.843 & & & 0.562 & 0.868 & \\
& Natural & 0.017 & 160.562 & 0.842 & & & 0.572 & 0.867 &  \\
& Random & 0.017 & 155.820 & 0.817 & & & 0.483 & 0.845 & \vspace{2mm} \\

\multirow{4}{*}{DenseNet-121}
& L-BFGS-B Sponge & 0.033 & 152.595 & 0.783 & & & 0.571 & 0.826 & \multirow{4}{*}{0.829} \\
& Sponge & 0.029 & 149.564 & 0.767 & & & 0.540 & 0.814 & \\
& Natural & 0.033 & 147.227 & 0.755 & & & 0.523 & 0.804 &  \\
& Random & 0.030 & 144.365 & 0.741 & & & 0.487 & 0.792 & \vspace{2mm} \\
% \multirow{3}{*}{GoogleNet}
% & EEE LBFGSB & 0.018 & 47.454 & 0.862 & 0.953 &   \\
% & EEE GA & 0.015 & 46.088 & 0.837 & 0.951 &   \\
% & Natural & 0.016 & 45.964 & 0.835 & 0.955 &   \\
% & Random & 0.015 & 44.164 & 0.802 & 0.938 & \vspace{2mm} \\

\multirow{4}{*}{MobileNet v2}
& L-BFGS-B Sponge & 0.011 & 87.511 & 0.844 & & & 0.692 & 0.890 & \multirow{4}{*}{0.996} \\
& Sponge & 0.010 & 84.513 & 0.815 & & & 0.645 & 0.868 & \\
& Natural & 0.011 & 85.075 & 0.821 & & & 0.646 & 0.873 & \\
& Random & 0.011 & 80.805 & 0.779 & & & 0.567 & 0.844 & \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Energy is reported in milli joules.
GA was ran for 100 epochs with a pool size of 100.
More results are available in Appendix.}
\label{tab:cv-bench}
\end{table*}



==> sections/tables/nlps_partial.tex <==
\begin{table*}[!h]
\centering
\begin{adjustbox}{scale=1.0,center}
\begin{tabular}{@{}lccccccccccc@{}}
\toprule
                & Input size & & $\text{NVML}_{\text{gpu}}$ & $\text{Natural}_{\text{asic}}$ & $\text{Random}_{\text{asic}}$ &
                & $\text{Sponge Mean}_{\text{asic}}$ & $\text{Sponge Top 10\%}_{\text{asic}}$ & & $\text{Energy}_{\text{gpu}}$ & $\text{Time}_{\text{gpu}}$ \\
\midrule
\multicolumn{11}{l}{\textit{\underline{Language Understanding: SuperGLUE Benchmark with \cite{liu2019roberta}}}} \vspace{3mm}\\
\multirow{3}{*}{CoLA}
& 15 & & 5829.32 & 4.30 & 69.72 & & 83.92 & 87.11 & & $\times20.25$ & $\times1.23$ \\
& 30 & & 9388.40 & 4.30 & 138.07 & & 164.07 & 169.91 & & $\times39.51$ & $\times1.48$ \\
& 100 & & 22698.87 & 4.30 & 452.49 & & 518.19 & 530.80 & & $\mathbf{\times123.42}$ & $\mathbf{\times3.82}$  \vspace{3mm}\\
\multirow{3}{*}{MNLI}
& 15 & & 6126.65 & 12.88 & 73.47 & & 86.97 & 89.96 & & $\times6.98$ & $\times1.32$ \\
& 30 & & 9631.68 & 17.66 & 142.63 & & 168.96 & 174.34 & & $\times9.87$ & $\times2.03$ \\
& 100 & & 22952.14 & 34.47 & 456.11 & & 518.89 & 531.40 & & $\mathbf{\times15.42}$ & $\mathbf{\times3.16}$ \vspace{3mm}\\
\multirow{3}{*}{WSC}
& 15 & & 27876.53 & 14.48 & 523.28 & & 1300.19 & 2152.67 & & $\times148.62$ & $\times9.83$ \\
& 30 & & 82822.58 & 34.94 & 1882.63 & & 3927.63 & 5348.06 & & $\times153.08$ & $\times19.25$ \\
& 100 & & 662811.96 & 194.89 & 16754.13 & & 25367.30 & 30692.95 & & $\mathbf{\times157.49}$ & $\mathbf{\times69.83}$ \vspace{3mm}\\
\midrule
\multicolumn{11}{l}{\textit{\underline{Machine Translation: WMT14/16 with \cite{ott2018scaling}}}}\vspace{3mm}\\
\multirow{2}{*}{En$\rightarrow$Fr}
& 30 & & 59597.32 & 31.87 & 109.80 & & 118.47 & 141.27 & & $\times4.43$ & $\times4.45$ \\
& 50 & & 93731.34 & 48.54 & 166.13 & & 249.89 & 569.85 & & $\times11.74$ & $\times13.51$ \vspace{3mm}\\
% Fr->En & & & & & & & & & \vspace{3mm}\\
\multirow{1}{*}{En$\rightarrow$De}
& 15 & & 18133.66 & 18.19 & 35.80 & & 242.39 & 542.35 & & $\times29.82$ & $\times32.86$ \\

\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Energy is reported in millijoules.
GA was ran for 100 epochs with a pool size of 100. We report GPU energy readings using NVML and show
the amount of energy and time increase as $\text{Energy}_{\text{gpu}}$ and
$\text{Time}_{\text{gpu}}$ respectively.
In addition, we show the performance of
samples from the evaluation dataset ($\text{Natural}_{\text{asic}}$),
random noise ($\text{Random}_{\text{asic}}$) and sponge example
performance on the accelerator simulator.
For sponge examples, we average the final GA pool samples and report it as
$\text{Sponge Mean}_{\text{asic}}$; in addition, the top $10\%$
sponge examples are averaged and reported as $\text{Sponge Top 10\%}_{\text{asic}}$.
More results are available in Appendix.}
\label{tab:nlp-bench}
\end{table*}


==> sections/tables/panelols.tex <==
\begin{table}
\begin{center}
\begin{tabular}{lclc}
\toprule
\textbf{Dep. Variable:}    &        engs        & \textbf{  R-squared:         }   &      0.9907      \\
\textbf{Estimator:}        &      PanelOLS      & \textbf{  R-squared (Between):}  &      0.9883      \\
\textbf{No. Observations:} &       83699        & \textbf{  R-squared (Within):}   &      0.9900      \\
\textbf{Date:}             &  Tue, May 12 2020  & \textbf{  R-squared (Overall):}  &      0.9900      \\
\textbf{Time:}             &      02:36:17      & \textbf{  Log-likelihood     }   &    -1.06e+06     \\
\textbf{Cov. Estimator:}   &       Robust       & \textbf{                     }   &                  \\
\textbf{}                  &                    & \textbf{  F-statistic:       }   &    2.163e+06     \\
\textbf{Entities:}         &         30         & \textbf{  P-value            }   &      0.0000      \\
\textbf{Avg Obs:}          &       2790.0       & \textbf{  Distribution:      }   &    F(4,80905)    \\
\textbf{Min Obs:}          &       2789.0       & \textbf{                     }   &                  \\
\textbf{Max Obs:}          &       2790.0       & \textbf{  F-statistic (robust):} &    1.274e+05     \\
\textbf{}                  &                    & \textbf{  P-value            }   &      0.0000      \\
\textbf{Time periods:}     &        2790        & \textbf{  Distribution:      }   &    F(4,80905)    \\
\textbf{Avg Obs:}          &       30.000       & \textbf{                     }   &                  \\
\textbf{Min Obs:}          &       29.000       & \textbf{                     }   &                  \\
\textbf{Max Obs:}          &       30.000       & \textbf{                     }   &                  \\
\bottomrule
\end{tabular}
\begin{tabular}{lcccccc}
                    & \textbf{Parameter} & \textbf{Std. Err.} & \textbf{T-stat} & \textbf{P-value} & \textbf{Lower CI} & \textbf{Upper CI}  \\
\midrule
\textbf{const}      &     4.552e+05      &     8.984e+04      &      5.0673     &      0.0000      &     2.792e+05     &     6.313e+05      \\
\textbf{temps}      &      -3149.0       &       1636.4       &     -1.9243     &      0.0543      &      -6356.3      &       58.413       \\
\textbf{rnd\_dummy} &      -1905.0       &       658.79       &     -2.8917     &      0.0038      &      -3196.2      &      -613.78       \\
\textbf{nat\_dummy} &      -79.079       &       653.54       &     -0.1210     &      0.9037      &      -1360.0      &       1201.9       \\
\textbf{times}      &     5.363e+07      &      7.53e+04      &      712.28     &      0.0000      &     5.349e+07     &     5.378e+07      \\
\bottomrule\\
\end{tabular}
\caption{Panel OLS on 10 natural, 10 random and 10 EEE samples on ResNet18}
\label{tab:panel_ols}
\end{center}
\end{table}
